A Control Theoretic Approach to Infrastructure-Centric Blockchain Tokenomics

There are a multitude of Blockchain-based physical infrastructure systems, operating on a crypto-currency enabled token economy, where infrastructure suppliers are rewarded with tokens for enabling, validating, managing and/or securing the system. However, today's token economies are largely designed without infrastructure systems in mind, and often operate with a fixed token supply (e.g., Bitcoin). This paper argues that token economies for infrastructure networks should be structured differently - they should continually incentivize new suppliers to join the network to provide services and support to the ecosystem. As such, the associated token rewards should gracefully scale with the size of the decentralized system, but should be carefully balanced with consumer demand to manage inflation and be designed to ultimately reach an equilibrium. To achieve such an equilibrium, the decentralized token economy should be adaptable and controllable so that it maximizes the total utility of all users, such as achieving stable (overall non-inflationary) token economies. Our main contribution is to model infrastructure token economies as dynamical systems - the circulating token supply, price, and consumer demand change as a function of the payment to nodes and costs to consumers for infrastructure services. Crucially, this dynamical systems view enables us to leverage tools from mathematical control theory to optimize the overall decentralized network's performance. Moreover, our model extends easily to a Stackelberg game between the controller and the nodes, which we use for robust, strategic pricing. In short, we develop predictive, optimization-based controllers that outperform traditional algorithmic stablecoin heuristics by up to $2.4 \times$ in simulations based on real demand data from existing decentralized wireless networks.

==> fig_latex/fig1_overview_diagram.tex <==
\begin{figure}[t]
    \includegraphics[width=1.0\columnwidth]{pics/fig1_BME_block_diagram.pdf}
    \vspace{-2em}
\caption{\small{\textbf{A Control System for Blockchain Token Economics:}
    We model a blockchain-based infrastructure network as a dynamical system, and design a controller (gray) to achieve a burn and mint equilibrium (BME). The controller takes in a forecast of consumer demand and node (supplier) growth, as well as the state of the treasury (blue). Then, it adaptively controls token payments $u^p_t$ and buy-backs $u^b_t$ to achieve a stable token price.
    \label{fig:tokenomics}
} }
    \vspace{-3em}
\end{figure}



==> fig_latex/fig2_game.tex <==
\begin{figure}[t]
    \includegraphics[width=0.5\columnwidth]{pics/fig2_game_formulation.pdf}
\caption{\small{\textbf{Strategic Pricing as a Game: } 
    In our game, the reserve (player 1) offers to buy-back tokens at the market price plus a bonus incentive of $\Delta p^t$ to reduce the circulating supply. However, the nodes (collectively, player 2) might want to only sell a fraction $\alpha_t$ of tokens since they could be valuable in the future. 
We solve this game using bi-level optimization methods, which results in an optimal strategy ($\Delta p_t^*$ and $\alpha^*$) for each player.
%We formulate a game between the reserve (player 1) and all token-owning nodes (collectively, player 2). The reserve offers to buy-back tokens at the market price plus a bonus incentive of $\Delta p^t$ to reduce the circulating supply. However, the nodes might want to only sell a fraction $\alpha_t$ of tokens since they could be valuable in the future. 
%However, if they refuse to sell back any tokens, the price might plummet due to an excess circulating token supply. 
    %and inflation.
    %We cast this game as bi-level optimization problem, which results in an optimal
    %strategy ($\Delta p_t^*$ and $\alpha^*$) for each player.
    \label{fig:game}
} }
\end{figure}



==> fig_latex/toy_example_caption.tex <==
\begin{figure}[t]
    \begin{minipage}[c]{0.35\textwidth}
        \includegraphics[width=\columnwidth]{pics/toy_example.jpg}
      \end{minipage}\hfill
      \begin{minipage}[c]{0.65\textwidth}
        \caption{\small{\textbf{Why Cooperate?}
          Consider a toy example with only 2 classes and 2 robots. The axes represent the number of data-points for each class. Our goal is to reach the target distribution (blue cross) where each class has 120 data-points, represented by $(120, 120)$. 
          The robots start at $(0,0)$ with no data-points in the cloud. The possible combinations that can be uploaded from robots 1 and 2 are shown as the shaded feasible action spaces (yellow and purple). This shaded region is 
          determined by the robot's local data distribution and vision model accuracy (Def. \ref{def:fspace}). \Greedy~ (black) individually calculates the projection of the target distribution onto each robot's feasible action space, but the sum of actions may not be optimal, leading to a high error (red). However, \Oracle~ accounts for the two robots' action spaces and thus minimizes the error between the target dataset and the sum of actions (grey). 
%between robots reduces our distance to the desired target distribution. 
        \label{fig:toy_ex}
    } }
    \end{minipage} 
\vspace{-1.5em}
\end{figure}


==> sections/bilevel.tex <==
As a cost function we will use quadratic cost function with respect to the price reference and thus the cost function becomes:

\begin{small}
    \begin{align}
        \cost = \frac{1}{2} \times \alpha \times (\tokenprice - \pricereference)^2
    \end{align}
\end{small}.

In here we will assume that the token holders are intelligent and they are aware of the controllers target and they are trying to maximize their utility in each time step.
so they select the maximium amount of token to sell in each time step to maximize their utility. Thus this problem can be posed as bilevel optimization problem. The controller problem is non-convex but coin holders problem is convex and we can solve it using the standard convex optimization techniques. for the optimal $\alpha$ we will assume that the KKT conditions hold.
Thus we can replace the controller problem with the following problem:

\begin{small}
    \begin{align}
        \min_{\incentive, \paytokens, \buybackdollars} &  c_f(p^{\text{Token}}_H) + \sum_{t=0}^H c_t(\tokenprice,\incentive,\paytokens,\buybackdollars) \\
        \text{s.t.} & S_{t+1} = \totalsupply + \buybacktokens - \paytokens  \forall \hspace{1mm} t = 0, \ldots, H-1  \\
        & R_{t+1}^{\text{Token}} = \tokenreserve + \paytokens - \buybacktokens \\
        & R_{t+1}^{\text{USD}} = \dollarreserve - \buybackdollars + \reserveincomes \\
        & \tokenprice = \frac{\demand}{\totalsupply} \\
        & \buybackdollars \geq 0 \\
        & \paytokens \geq \frac{\beta_t \times \reserveincomes}{\tokenprice} \\
        & \buybacktokens \leq \alpha \times \totalsupply \times (\tokenprice + \incentive) \\
        & \lambda_i \geq 0 \\
        & \lambda_1 \times (1-\alpha) = 0 \\
        & \lambda_2 \times (-\alpha) = 0 \\
        & \alpha \geq 0 \\
        & \alpha \leq 1 \\ 
        & \Delta_\alpha \utility - \lambda_1 - \lambda_2 = 0 \\ 
    \end{align}
\end{small}.

Which we can solve with sequential convex programming (SCP). Therefor we can solve the bilevel optimization problem with the following steps:

\begin{algorithm}[H]
\caption{Bilevel Optimization Problem}
\label{alg:scp}
\begin{algorithmic}[1]
\STATE \textbf{Input:} $H$, $\alpha$, $\beta$, $\gamma$, $\pi$, $\tokenprice$, $\pricereference$, $\reserveincomes$, $\reservepayments$, $\numconsumer$, $\numproducer$, $\productprice$, $\tokenreserve$, $\dollarreserve$, $\totalsupply$
\STATE \textbf{Output:} $\incentive$, $\paytokens$, $\buybackdollars$
\STATE \textbf{Initialize:} $\alpha = 0.5$, $\lambda_1 = 0$, $\lambda_2 = 0$
\STATE \textbf{for} $t = 0$ \textbf{to} $H$ \textbf{do}
\STATE \hspace{1mm} $\lambda_1 = \lambda_1 + \alpha \times \Delta_\alpha \utility$
\STATE \hspace{1mm} $\lambda_2 = \lambda_2 - \alpha \times \Delta_\alpha \utility$
\STATE \hspace{1mm} $\alpha = \alpha + \lambda_1 \times (1-\alpha) + \lambda_2 \times (-\alpha)$
\STATE \hspace{1mm} $\alpha = \max(0, \min(1, \alpha))$
\STATE \hspace{1mm} $\Delta_\alpha \utility = \frac{1}{2} \times \alpha \times (\tokenprice - \pricereference)^2$
\STATE \hspace{1mm} $\incentive = \alpha \times \Delta_\alpha \utility$
\STATE \hspace{1mm} $\paytokens = \frac{\beta_t \times \reserveincomes}{\tokenprice}$
\STATE \hspace{1mm} $\buybackdollars = \alpha \times \totalsupply \times (\tokenprice + \incentive)$
\STATE \hspace{1mm} $\buybacktokens = \buybackdollars \times \frac{\tokenreserve}{\dollarreserve}$
\STATE \hspace{1mm} $\tokenreserve = \tokenreserve + \paytokens - \buybacktokens$
\STATE \hspace{1mm} $\dollarreserve = \dollarreserve - \buybackdollars + \reserveincomes$
\STATE \hspace{1mm} $\totalsupply = \totalsupply + \buybacktokens - \paytokens$
\STATE \hspace{1mm} $\tokenprice = \frac{\demand}{\totalsupply}$
\STATE \hspace{1mm} $\pricereference = \pi \times \tokenprice$
\STATE \hspace{1mm} $\reserveincomes = \gamma \times \reservepayments$
\STATE \hspace{1mm} $\reservepayments = \numconsumer \times \productprice + \numproducer \times \tokenprice$
\STATE \hspace{1mm} $\demand = \numconsumer \times \productprice + \numproducer \times \tokenprice$
\STATE \textbf{end for}
\end{algorithmic}
\end{algorithm}


==> sections/discussion.tex <==
\textcolor{red}{Future Work:
    \begin{itemize}
\item Investigating implementation (i.e. decentralization through multiparty computation, communication complexity tradeoffs, etc.
        \item Alternative solutions to game theoretic extension
    \end{itemize}
}


==> sections/old/abstract.tex <==
Today, we are seeing a surge in blockchain-based physical infrastructure networks, ranging from decentralized 5G wireless to electric vehicle charging networks. 
These networks operate on a crypto-currency based token economy, where node suppliers are rewarded tokens for building and securing the network. However, today's token economies largely target decentralized finance and often operate with a fixed token supply (e.g., Bitcoin). Such fixed supply systems often encourage early adopters to hoard valuable tokens, thereby dis-incentivizing new nodes from joining or maintaining the network. 
We argue that token economies for infrastructure networks should be radically different -- they should 
\textit{continually incentivize} new suppliers to join the blockchain and provide ubiquitous services, such as 5G connectivity. 
%We argue that a token economy for infrastructure networks should \textit{continually incentivize} new suppliers to join the blockchain and provide ubiquitous services, such as 5G connectivity. 
As such, the token rewards should gracefully scale with the size of the blockchain, but should be delicately balanced with consumer demand to avoid inflation. 
To achieve such an equilibrium, the blockchain's token economy should be \textit{adaptable} and controllable so that it maximizes the total utility of all users, such as achieving a stable, steadily growing token price. 
As such, our key contribution is to model token economies as \textit{dynamical systems} -- 
the circulating token supply, price, and consumer demand change as a function of how much we pay nodes and charge consumers for infrastructure services. Crucially, this dynamical systems view allows us to leverage powerful tools from mathematical control theory to maximize a blockchain network’s performance. We develop predictive, optimization-based controllers that outperform traditional algorithmic stablecoin heuristics by up
to \SC{X $\times$} in simulations that use real demand data from operational decentralized wireless networks.

%Moreover, we show the benefits of optimal control in simulations that use real demand/growth patterns from operational decentralized wireless networks.

%Our central thesis is that the blockchain's token economy should be \textit{adaptable} and controllable so that it maximizes the total utility of all users, such as achieving a stable, steadily growing token price. 

%real node/consumer demand patterns from operational DeWi networks. 
%However, token economies for infrastructure networks can be starkly different from traditional financial networks, which often operate with a fixed supply of tokens (e.g., Bitcoin). Such fixed supply systems often 
%Many of today's token economies, such as Bitcoin, operate with a fixed token supply, which often encourages early adopters to hoarde valuable tokens, which in turn dis-incentivizes new nodes from joining or maintaining the network. 
%Specifically, our key contribution is to model token economies as \textit{dynamical systems},
%which allows us to leverage powerful tools from mathematical control theory to maximize a blockchain network’s utility function. 
%
%
%
%
%model predictive controllers (MPC) for the token economy 
%
%Control theory is a natural tool since the token economy is a dynamical system – the circulating token supply and token price change as as a function of how we pay token rewards to nodes and buy tokens from consumers in exchange for network services. 
%
%, and consumer demand change as a function of how we
%
%our burn and mint decisions. Likewise, we have control authority – we can adapt how we burn or mint to regulate the token economy. Moreover, we can design a control cost function that captures key metrics for desired blockchain performance and evolution of the blockchain dynamical system. Crucially, we can model the dynamics of the system, since we engineer the blockchain protocol and token economy dynamics. As such, regulating the blockchain token economy is a model-based control problem, which can be solved using powerful ideas from nonlinear optimization and optimal control theory. 
%
%
%
%
%Since the state of the network changes over time, our key inisg
%
%
%Our key contribution is to design token economies for infrastructure networks that are adaptive and gracefully scale with growing node and consumer adoption. To do so, we model
%
%
%
%
%
%However, the size of the continually growing blockchain
%To address this concern, several recent projects propose a ``burn-and-mint'' tokenomics model, where we mint new tokens to reward nodes, while tokens are ``burnt'' (deleted from the circulating supply) when consumers demand network services. However, the stability 
%
%lead to inflation if such payments are not delicately balanced with the consumer demand for infrastructure services. To solve such problems, a number of projects have recently proposed a “burn-and-mint” tokenomics model, where a central reserve “mints” tokens to reward suppliers, while tokens are “burnt” (deleted from the circulating supply) when consumers want to use network services. By adaptively burning tokens, we can reduce the token supply to reach a supply and demand equilibrium. 
%
%
%for Helium or even electric charging stations for Tesla’s new TeslaCoin. 
%As such, the number of tokens should gracefully scale with the size of the blockchain network, which we cannot know a-priori. However, continually rewarding suppliers with newly created tokens can lead to inflation if such payments are not delicately balanced with the consumer demand for infrastructure services. To solve such problems, a number of projects have recently proposed a “burn-and-mint” tokenomics model, where a central reserve “mints” tokens to reward suppliers, while tokens are “burnt” (deleted from the circulating supply) when consumers want to use network services. By adaptively burning tokens, we can reduce the token supply to reach a supply and demand equilibrium. 
%
%
%Our central thesis is that BME needs to be “programmable” so that  blockchain-based infrastructure networks can maximize the total utility of all users. 
%
%For example, this network utility function (performance criterion) can include maintaining a stable, steadily growing token price with low volatility. Likewise, this network cost function can incentivize new suppliers/consumers to expand geographical coverage. Moreover, the BME-based token economy might always need to satisfy strict performance guarantees and constraints. For example, we might limit the number of tokens minted or burned per day or always need to keep a minimum amount of tokens in a central treasury. 
%
%Our key insight is that token economies can be modeled as dynamical systems, which allows us to leverage powerful ideas from mathematical control theory to maximize a blockchain network’s utility function. Control theory is a natural tool since the token economy is a dynamical system – the circulating token supply, token price, and consumer demand change as a function of our burn and mint decisions. Likewise, we have control authority – we can adapt how we burn or mint to regulate the token economy. Moreover, we can design a control cost function that captures key metrics for desired blockchain performance and evolution of the blockchain dynamical system. Crucially, we can model the dynamics of the system, since we engineer the blockchain protocol and token economy dynamics. As such, regulating the blockchain token economy is a model-based control problem, which can be solved using powerful ideas from nonlinear optimization and optimal control theory. 
%
%
%
%
%
%- central need to create a token economy that incentivizes suppliers to build etc the network and likewise incentivizes demand for infra services from consumers
%
%Today, we 
%
%
%such as Bitcoin
%
%These networks reward infrastructure nodes (suppliers) 
%
%
%
%Likewise, consumers of network services buy and remove tokens ("burn") from the circulating supply to use infrastructure services. 
%
% in order to pay suppliers to build and validate the network
%
%
%Decentralized wireless (Helium, Pollen)
%Tesla Coin (Electric Vehicle Charging)
%FileCoin etc. 
% 
%


==> sections/old/circ_supply.tex <==
Naturally, paying tokens out of the reserve increases supply, whereas buying tokens back to place in the reserve decreases supply.
Therefore, the circulating supply $S_t$ at any time $t$, along with the number of tokens paid out to service providers from the reserve and the number of tokens bought back to place into the reserve, determines the circulating supply for the next timestep.
This is given symbollically by,
\begin{small}
\begin{equation}\label{eq:supply}
    S_{t+1} = \totalsupply + \underbrace{\paytokens}_{\text{Tokens Paid}} - \underbrace{\buybacktokens}_{\text{Tokens Bought Back}},
\end{equation}
\end{small}
where the units for $\paytokens$ and $\buybackdollars$ are in tokens and dollars respectively.
Specifically, while $\paytokens$ is the number of tokens paid out to the service providers from the reserve in timestep $t$, $\buybackdollars$ is the number of dollars the controller pays to the users to purchase their tokens.
This means the number of tokens bought back in time $t$ is $\buybackdollars$ divided by the purchasing price $(\tokenprice + \incentive)$.
We define $\tokenprice$ as the current market price of the token, while $\incentive$ is the extra amount the controller pays the users over the market price so as to incentivize them to part with their tokens.
If the token owners are not rational, $\incentive$ simply equals zero.
However, a rational owner may not part with their tokens if they believe the price will increase in successive timesteps, and so the controller needs to pay the extra incentive price $\incentive$ to overcome the agent beliefs.
We formulate a mathematical game to calculate $\incentive$ for rational agents in Section \ref{sec:game}.


==> sections/old/conclusion.tex <==
The central thesis of this paper is that blockchain token economies should be programmable
and dynamically adapt to node growth and consumer demand. Our key contribution is to model
a token economy as a controlled dynamical system, which allows us to leverage rigorous systems theory to design token economies that meet high-level performance metrics (network cost functions). 
We believe our work is timely as several blockchain projects are adopting burn and mint strategies and our novel framework allows us to (a) explicitly prove these systems reach a stable equilibrium and (b) flexibly steer this equilibrium to incentivize stable network growth. We are working with several blockchain projects to instantiate these ideas in practice, which we hope to report on in future work.



==> sections/old/discussion.tex <==
\textcolor{red}{Future Work:
    \begin{itemize}
\item Investigating implementation (i.e. decentralization through multiparty computation, communication complexity tradeoffs, etc.
        \item Alternative solutions to game theoretic extension
    \end{itemize}
}


==> sections/old/experiments.tex <==
The goal of our evaluation is to show that (i) using control theory allows us to achieve a more stable, increasing token price and (ii) we can reduce control cost using an optimization-based controller instead of a reactive PID controller. Thus, we now describe our benchmark algorithms and evaluation metrics. 

\paragraph*{Evaluation Metrics and Benchmark Algorithms: }

We compare treasury controllers on the following metrics: 

\begin{enumerate}
    \item \textbf{Stable Token Price}: We report whether the token price is increasing, its volatility, and the mean squared error (MSE) from a reference price trajectory.
    \item \textbf{Control Cost}: We report the control cost $J$, which is a weighted sum of the tracking error (MSE between the token price and time-variant reference price) as well as control effort (how many tokens are burned at each time-step).
\end{enumerate}

We report these metrics for various realistic scenarios where (i) the supply of hotspots out-paces the consumer demand, (ii) the supply and demand roughly match, and (iii) the supply lags the consumer demand. Further, we plot a distribution of control cost over many scenarios and initial conditions (starting token supplies) to emulate the controller in various scenarios. Our experiments compare the following schemes: 

\begin{enumerate}
	\item \textbf{Model Predictive Control (MPC)}: This is our proposed scheme, where the controller receives a stochastic forecast of node supply and consumer demand. The controller's optimization problem  aims to find a finite sequence of controls to minimize the control cost, which exploits the token economy's model-based dynamics outlined earlier. If we have nonlinear dynamics and a quadratic approximation of control cost, but no strict state or control constraints, we can use the iterative Linear Quadratic Regulator (iLQR) controller. Likewise, if we have strict control constraints, we use Sequential Convex Programming (SCP), specifically Sequential Quadratic Programming (SQP).
	\item \textbf{Proportional Integral Derivative (PID)}: PID is a common benchmark in the control systems community, and is widely used in industrial systems such as cruise control, robotic manipulators, and in some algorithmic stablecoins. However, PID does not explicitly optimize for a high-level cost function like MPC.
	\item \textbf{No Control}: We consider the worst case where no adaptive control is implemented in the token economy. 
\end{enumerate}

\subsection{Experiment Design}
First, we evaluate our control system on synthetic node supply and consumer demand growth data. Then, we repeat our simulations with real-world timeseries of supply/demand from the Helium DeWi network.

In all experiments, we have a timeseries of the number of nodes $n_t$ and devices $d_t$. Then, given a noisy forecast of the supply/demand growth for a horizon of $H$ future steps, we implement the various control benchmarks starting with different initial conditions $x_0$ representing the starting token supply etc. Then, we visualize the resulting token supply $s_t$ and token price $p_t$ compared to the desired reference trajectory, as shown in Fig. XYZ. Finally, we report a distribution of
control costs across various timeseries patterns in the boxplots in Fig. ABC.

\subsubsection{Synthetic Experiments}

Our synthetic experiments aim to generate realistic supply/demand growth patterns with additive, zero-mean Gaussian noise. For example, we use a sigmoidal growth pattern where demand and supply rapidly rise during the middle of network adoption, but slowly taper off. We also simulate a logarithmic growth function where the nodes/consumers steadily grow over time.

Each simulation trial has a different reference token supply, which could be constant to emulate a standard ``fixed-supply'' tokenomics scheme or vary over time to allow a stable price growth, such as a logarithmic reference price trajectory. In each trial, the initial token supply $s_0$ is randomly chosen away from the reference, and we evaluate the ability of the controller to dynamically regulate the system. 

\textbf{Does MPC outperform benchmarks to yield a stable token price growth?}
Fig. ABC shows an example trajectory of our system. The exogenous growth of supply and demand is shown in the top left. Since the number of nodes quickly grows compared to consumers, we mint a significant amount of tokens to reward nodes, which increases the circulating token supply. Since the demand is relatively low, this scenario can lead to inflation and a dropping token price, which occurs without any control (blue). However, we can see both our MPC controller and PID adaptively curb
the number of miner token payments and selectively buy back tokens from the circulating supply, which curtails the number of cirulating tokens. As a result, the token price stably increases over time. However, MPC explicitly optimizes for the reference tracking cost function as opposed to PID, which allows it to more accurately track the reference.

\textbf{Does MPC reduce control cost compared to heuristic controllers?}
We now evaluate our ultimate performance metric, the control cost, across a wide variety of growth patterns and initial conditions. Specifically, we used 3 growth patterns with Gaussian noise (sigmoidal, logarithmic, exponential) and many scenarios where demand outstrips supply and vice versa. Fig. AXB shows the overall control cost, tracking error, and control effort for all 3 benchmarks. Clearly, MPC achieves a lower control cost than the PID heuristic (Wilcoxon p-value of ABC is
statistically significant at the $0.05$ level). As shown in Fig. ABC, the key reason for this difference is that PID is largely \textit{reactive} -- it proportionally responds to the current error and integrates the cumulative error, but does not forecast the future system state accurately to optimize performance. In stark contrast, MPC explicitly solves an optimization problem to minimize the control cost over the forecast horizon $H$, implements the first control, and re-plans
to react to estimation errors, which improves ultimate performance.

\subsubsection{Simulations from Real DeWi Network Data}
We now repeat the same experimental procedure, but with real timeseries of node growth $n_t$ and consumer growth $d_t$ from the Helium DeWi network. At the time of writing, the Helium network uses a BME protocol and has approximately $N$ geo-distributed nodes and $D$ devices. First, since the Helium growth patterns are smooth, we use a classical Auto-Regressive Integrated Moving Average (ARIMA) forecasting model to predict network growth $H=ZYZ$ days in advance. Then, we
implement our controller on a distribution of scenarios with different reference price trajectories. Our results in Figs. A and B indicate that MPC outperforms the benchmarks and reduces the control cost compared to PID in a statistically significant manner. 

\subsection{Limitations}
Our trace-driven simulations are limited by offline, historical Helium DeWi data. However, the growth of nodes and consumers might significantly deviate from historical patterns if we actually implemented our proposed controller in the network. In future work, we plan to answer such ``what-if'' questions using recent advances in counterfactual analysis \cite{morgan2015counterfactuals,pearl2010causal} and synthetic interventions
\cite{agarwal2020synthetic}. Further, we are actively working with operational infrastructure blockchains to deploy our control strategies. 




==> sections/old/intro.tex <==

\iffalse
The ability to hold valuable assets and spend those assets on goods and services constitute two key features of a healthy economic system.
Designs of early cryptocurrencies emphasized the former, focusing on creating deflationary assets via scarcity.
These designs have attracted speculative behavior which in turn has induced volatility in the value of these assets.
While attractive to investment traders, these dynamics do not bode favorably in the facilitation of payments for goods and services using these cryptocurrencies.
Namely, the risk involved in receiving payment which may quickly lose value is too large to ignore for most service providers.
Moreover, this risk goes both ways as consumers may also be hesitant to pay the service provider today, in the presence of the belief that the value of their holdings will increase tomorrow.
Therefore, many traditional cryptocurrencies do not support our second feature of a healthy economic system: The ability to freely spend assets on goods and services.

To solve this problem, {\em stable coins} have been touted as a solution (see \cite{moin2020sok} for a comprehensive survey).
Stable coins are cryptocurrencies whose values are ``pegged'' to some reference point.
Specifically, this is typically accomplished either by holding collateral or through algorithmic solutions.
On the one hand, collateral based methods are simple and well understood, while on the other hand such methods centralize the power and responsibility of maintaining the token's value into the collateral holder.
This invites deceptive behavior, as was seen when Tether, a popular collateral backed stable coin, openly admitted that it was only 74\% collateralized after claiming it was collateralized in full \cite{affidavit}.
Moreover, this sort of system relies on the collateral holder to have enough assets to float the stable coin through long periods of dips, which must end when the funds run out.
Algorithmic solutions pose an alternative to backing with collateral.
Specifically, algorithmic stable coins strategically control the supply and stabilize the price in periods of demand dips and valleys.
Particulary interesting are systems implementing {\em burn and mint} models.
One example is Helium network, which is an algorithmic stable coin system for decentralized wireless networks.
Users {\em burn} a native token, HNT, to obtain data credits which can be used to obtain wireless services.
{\em Minting} occurs by the network protocol paying the service providers for the coverage they provide to the users.
The rate of minting is controlled heuristically to stabilize the conversion rate between HNT and data credits, which has lead some to refer to the resulting saddle point as a {\em burn and mint equilibrium}.
Furthermore, in contrast to collateral based systems this method is more decentralized as it is based off of controlling market dynamics and does not require central holdings.

In spite of their positive traits such burn and mint systems are not well understood.
Moreover, their control strategies are heuristic and reactive where it may be possible to be methodological and predictive.
For this reason, we investigate burn and mint systems through the lens of optimal control theory.
In particular, in discrete rounds suppose that we are given a forecast of the demand for the next time step.
Then, in each time step we wish to use this forecast to minimize the error between the price of a token and a fixed reference point.
We formulate this as a model predictive control problem, and investigate optimal policies therein.
Furthermore, our formulation is flexible enough to accomodate extra constraints, and we extend our model to factor in rational behavior in the token holders induced by their beliefs about the trajectory of the token price.

\input{fig_latex/fig1_overview_diagram.tex}

Beginning in Section \ref{sec:model}, we formally pose the problem.
In particular, we identify the dynamics of burn and mint systems a describe an adaptive controller stabilizing the token price.
In Section \ref{sec:method}, we continue by relaxing our controller into a sequential convex program and show how to solve the relaxation with iterative quadratic regulator methods.
We move on to considering the effects of rational behavior in the token holders in Section \ref{sec:game}.
Specifically, our method requires the ability to buy back tokens from token holders to manipulate the supply.
If the token holders are rational then it is possible that they may not wish to sell if they believe their tokens will accumulate in value.
To offset this our controller pays an extra ``incentive price'' during buybacks.
We formulate this setting as a bilevel optimization problem, where the inner level corresponds to the token holders fixing their strategy and the outer level corresponds to the controller responding to it.
Finally, in Section \ref{sec:experiments} we overview our empirical findings when applying our methods to simulated markets, before finishing with discussions and future work in Section \ref{sec:discussion}.
\fi
\subsection{Related Work}

We are not the first to model Blockchain systems as a dynamical system, notable examples are \cite{zargham2018state,zhang2020modeling,caginalp2018dynamical}.
However, even these research efforts steer their focus towards how aspects such as miner profitability and block rewards influence supply and demand dynamics.
Even though these works touch on service based economies, such as those we focus on, our work differs in that our formulation of a dynamical system is specific to the enablement of model predictive control.
Specifically, in our model the supply is fully specified by the actions of the controller, while the demand is specified via forecasts.
Thus, our controller specification is decoupled from the possibly complex trajectory of the demand, and the strength of our controller's predictions is tied to the strength of the forecasts used in the system.

In order to strengthen the robustness of our methods we also consider the effects of rational behavior on the part of the consumers in the system.
Of course, we are also not the first to employ game theoretic analyses in Blockchain systems which have a long legacy going back to the original Bitcoin whitepaper \cite{nakamoto2008bitcoin}.
Since the discovery of the selfish mining attack \cite{eyal2018majority}, game theoretic methods have been used to investigate rational deviations \cite{carlsten2016instability}, mining pools \cite{eyal2015miner}, and more recently transaction fee auctions in Ethereum like blockchains \cite{roughgarden2021transaction,chung2021foundations}.
Our work is not directly related, however, as our focus is on the effects of rational behavior on buy-back and pay strategies used to stabilize token prices, and not necessarily on the effects to an underlying Blockchain protocol.

Finally, as our aim is to stabilize a token price in a Blockchain network our work is somewhat related to algorithmic stable-coins.
However, it must be noted that our interests are in intelligently controlling the circulating supply of a token to balance the increasing payments to service providers needed to scale a network with a prespecified control trajectory on the token price.
In that sense, our work is more related to service networks employing burn and mint systems such as Helium \cite{haleem2018decentralized} (which inspired our model) and Factom \cite{snow2014factom} than more general purpose stable-coins like Reflexer \cite{RAI} or Terra \cite{kereiakes2019terra}.
Furthermore, these works are {\em reactive} through the use of heuristic methods such as PID, whereas our work is {\em predictive} through optimal adaptive control methods.
And as our focus is on service providing networks, our work is immediately to applicable not only to the DeWi scenarios like Helium \cite{haleem2018decentralized} or 5G networks \cite{messie2019baladin}, but also to file sharing \cite{filecoin}, electric vehicle charging, and decentralized video streaming \cite{petkanics2018protocol}.



==> sections/old/methodology.tex <==
\textcolor{red}{showing how to relax problem (\ref{eq:formal_problem}) and solve with iLQR/SCP should go here.}


==> sections/old/preamble.tex <==



\usepackage{nicefrac}
\usepackage{url}
\usepackage{subfig}
\usepackage{multirow}
\usepackage{bbold}
\usepackage{balance}


\usepackage{footnote}
\usepackage{epsfig}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{relsize}


\usepackage{stackengine}
\usepackage{algorithmic,comment}
\usepackage[ruled,vlined,commentsnumbered,titlenotnumbered,linesnumbered]{algorithm2e}
\usepackage{float}

\usepackage[font=small,labelfont=bf]{caption}



\usepackage{colortbl}
\usepackage{url}
\usepackage{color}

\newcommand{\SC}[1] {{\color{blue} #1}}


\newcommand{\productprice}{p^{\text{prod}}_t}
\newcommand{\numconsumer}{n_t}
\newcommand{\numproducer}{d_t}
\newcommand{\totalsupply}{S_t}
\newcommand{\tokenreserve}{R^{\text{Tok}}_t}
\newcommand{\dollarreserve}{R^{\text{USD}}_t}
\newcommand{\buybackdollars}{u^{\text{B}}_t}
\newcommand{\paytokens}{u^{\text{P}}_t}
\newcommand{\demand}{D_t}
\newcommand{\tokenprice}{p^{\text{Tok}}_t}
\newcommand{\pricereference}{p^{\text{ref}}_t}
\newcommand{\reserveincomes}{\text{Inc}_t}
\newcommand{\reservepayments}{\text{Pay}_t}
\newcommand{\incentive}{\Delta p_t}
\newcommand{\buybacktokens}{\frac{u^{\text{B}}_t}{\tokenprice + \incentive}}
\newcommand{\state}[1]{x_{#1}}
\newcommand{\control}[1]{u_{#1}}
\newcommand{\cost}[1]{c_{#1}}
\newcommand{\forecasted}[1]{s_{#1}}
\newcommand{\statespace}{\mathcal{X}}
\newcommand{\controlspace}{\mathcal{U}}
\newcommand{\utility}{U_t(\alpha,\incentive)}


% math
\newcommand{\reals}{\mathbb{R}}
\newcommand{\realsplus}{\mathbb{R}_{+}}







==> sections/old/primer_control.tex <==
We now introduce several state-of-the-art control methodologies and how they can be used for blockchain tokenomics. The state vector is denoted by $x_t \in \reals^n$, the control vector by $u_t \in \reals^m$, and the dynamics are given by $x_{t+1} = f(x_t, u_t; s_t)$, where $s_t$ is an exogenous timeseries input, such as a demand forecast. Since we have forecasts of node and consumer growth for $H$ steps in the future, we naturally have a finite horizon control problem of $H$ steps. Our
goal is to optimize the performance metric, which is to minimize the aggregate control cost $J$. 
Typically, the control cost $J$ is a sum of a terminal cost and stage costs penalizing state deviations from a reference trajectory (tracking error) and control effort, of the form $J = c_H(x_H) + \sum_{t=0}^{H} c_t(x_t, u_t)$, where $c_t()$ is a possibly time-variant cost. 

Crucially, we have a good nominal model of the dynamics, since the token economy is under our design. Of course, there are uncertainties which arise due to the stochastic demand forecast. Since we have known nominal dynamics, we use standard \textit{model-based} control techniques, which solve an optimization problem to find the optimal set of controls to minimize the cost function subject to dynamics constraints
\cite{Camacho2013,borrelli2017predictive}. We now outline these methods as they apply to our tokenomics
problem. 

\textbf{Iterative Linear Quadratic Regulator (iLQR): } 
A canonical model in optimal control is the linear quadratic regulator (LQR), where we have linear dynamics and a quadratic cost function that weights state tracking error and control effort, such as energy expenditure \cite{aastrom2021feedback}. The linear dynamics are given by $x_{t+1} = A_t x_t + B_t u_t$ and the cost function is given by $J(u_{0:H-1}; x0) = x_H^T Q_H x_H + \sum_{t=0}^H x_t^T Q_t x_t + u_t^T R_t u_t$, where all $Q_t$ are positive semi-definite matrices and $R_t$ are positive definite to ensure non-negative costs. 
The optimal solution to LQR is an affine state feedback controller of the form $u^{*}_t = K_t x_t + k_t$, where $K_t$ and $k_t$ are obtained via dynamic programming and the discrete Algebraic Ricatti Equation. Alternatively, LQR can be solved as a convex program, specifically a quadratic program (QP) \cite{boyd2004convex}.

In practice, we want our system to follow a non-zero reference trajectory given by $(\bar{x}_t, \bar{u}_t)$, such as regulating the system to track a time-varying token supply. Moreover, the dynamics $f_t(x_t, u_t)$ could be non-linear and the cost function $c_t(x_t, u_t)$ could be non-convex nor quadratic. The key insight behind \textit{iterative} LQR or iLQR \cite{van2014iterated} is that we can \textit{linearize} a system's nonlinear dynamics around the reference trajectory $(\bar{x}_t,
\bar{u}_t)$ if the dynamics are differentiable. Thus, if we compute the Jacobian matrix of the nonlinear dynamics anchored at the current reference $\bar{x}_t, \bar{u}_t$, we obtain the dynamics matrix $A_t = \frac{\partial f_t}{\partial x}(\bar{x}_t, \bar{u}_t)$ and control matrix $B_t = \frac{\partial f_t}{\partial u}(\bar{x}_t, \bar{u}_t)$. Likewise, for a twice continuously differentiable cost function, we can form a local quadratic approximation of the cost function using the Taylor Series
expansion: \SC{XYZ}.

Given a nominal reference trajectory, linearized dynamics, and a quadratic approximation of the cost, we can simply invoke LQR to improve our nominal reference trajectory. The process repeats until the control cost converges, which is analagous to Newton's method. Crucially, iLQR is our solution method of choice for our tokenomics problem, since we have smooth nonlinear dynamics, a quadratic cost function, and a well defined reference trajectory for the token price/circulating
supply.

\textbf{Sequential Convex Programming (SCP): }
Sequential Convex Programming extends the core ideas behind iLQR to control problems with strict state or control constraints \cite{bonalli2019gusto,malyuta2021convex}. First, we linearize the dynamics around a reference trajectory, just as in iLQR. Then, we form a convex approximation of the cost function, often using a local quadratic approximation. Thus, we recover a convex optimization problem with state/control constraints, which we solve to obtain a new nominal trajectory. We then find a new convex relaxation of the original
problem around the updated nominal trajectory and repeats until the control cost saturates. 
We refer the reader to \cite{malyuta2021convex,tassa2012synthesis} for a detailed discussion of iLQR and SCP.

\textbf{Proportional Integral Derivative (PID) Control: }
Our proposed solution uses iLQR and SCP because we can model the token dynamics and explicitly want to optimize a cost function. We compare these methods to a benchmark proportional integral derivative (PID) controller. PID controllers are often used in compute-constrained, linear control systems to achieve stability \cite{aastrom2021feedback}. However, they do not explicitly optimize a cost function like iLQR/SCP, and often require extensive tuning and can overshoot a reference trajectory. PID is a fitting
benchmark due to its simplicity and the fact that recent algorithmic stablecoins, such as the RAI index \cite{RAI}, use PID.

A PID controller operates on an error signal, which penalizes the deviation of the current state and desired/reference state. In our setting, the error signal is the difference between the reference token supply $S^\mathrm{ref}_t$ and actual, measured token supply $S_t$. Then,  a PID controller generates a control decision $u_t$ that is proportional to the instantaneous error (P term), integrates past errors (I term), and forecasts how the error will change (derivative, D term) as
follows: $u_t = k_p (S^{\mathrm{ref}}_t - S_t) + k_i \sum_{k=0}^{t-1} (S^{\mathrm{ref}}_t - S_t) + k_d (S^{\mathrm{ref}}_{t+1} - S_{t+1})$.




==> sections/old/problem_statement.tex <==
In this section we introduce our dynamical system model for token dynamics in infrastructure networks, along with our formal control problem.
Ultimately, our goal is to develop the quantities that will serve as the state and control variables, as well as sensible cost functions for our controller.
In what immediately follows, we expouse the details of the underlying dynamical system in Section \ref{subsec:token_dynamics}.
Namely, we show the relationships between the token's circulating supply, price, and reserve used by the controller.
We will see that these components will form our state variables which are controlled via buying back tokens and paying tokens to the user base.
Following this, in Section \ref{subsec:control_problem} we fully make this connection by posing our formal control problem, which we examine and relax in subsequent sections.

\subsection{The Token Economy as a Dynamical System}\label{subsec:token_dynamics}

In examining the token economy, we assume that it is a closed system, meaning that the power to change the circulating supply is endowed only in the buyback and pay mechanism and no exogenous actor. 
Really, this amounts to saying that no user will intentionally burn their own tokens and lose assets.
Furthermore, we examine the token economy as a discrete time system.

\subsubsection{Circulating Supply}

Naturally, paying tokens out of the reserve increases supply, whereas buying tokens back to place in the reserve decreases supply.
Therefore, the circulating supply $S_t$ at any time $t$, along with the number of tokens paid out to service providers from the reserve and the number of tokens bought back to place into the reserve, determines the circulating supply for the next timestep.
This is given symbollically by,
\begin{equation}\label{eq:supply}
    S_{t+1} = \totalsupply + \underbrace{\paytokens}_{\text{Tokens Paid}} - \underbrace{\buybacktokens}_{\text{Tokens Bought Back}},
\end{equation}
where the units for $\paytokens$ and $\buybackdollars$ are in tokens and dollars respectively.
Specifically, while $\paytokens$ is the number of tokens paid out to the service providers from the reserve in timestep $t$, $\buybackdollars$ is the number of dollars the controller pays to the users to purchase their tokens.
This means the number of tokens bought back in time $t$ is $\buybackdollars$ divided by the purchasing price $(\tokenprice + \incentive)$.
We define $\tokenprice$ as the current market price of the token, while $\incentive$ is the extra amount the controller pays the users over the market price so as to incentivize them to part with their tokens.
In the case that the users are not rational, $\incentive$ simply equals zero.
However, a rational user may not wish to part with their tokens if they believe the price will increase in successive timesteps, and so the controller needs to pay the extra incentive price $\incentive$ to overcome the agent beliefs.
In the presence of rational agents, $\incentive$ can be calculated by examining an associated simultaneous game.
We more fully examine the details of this in the sequel.

\subsubsection{Reserve}

The controller will hold two reserves, one being comprised of tokens and the other dollars. 
At time $t$, the values of these reserves are given by $\tokenreserve$ and $\dollarreserve$ respectively.
The dollar reserve increases with the income received from users purchasing tokens, and decreases with buy backs from the market.
Symbolically, this is,
\begin{equation}\label{eq:reserve_dollars}
    R_{t+1}^{\text{USD}} = \dollarreserve - \buybackdollars + \reserveincomes,
\end{equation}
where $\buybackdollars$ is the dollars used to buy back tokens in time $t$ (as mentioned before), while the new variable $\reserveincomes$ is the income received from users purchasing tokens.
Furthermore, we make the assumption that $\reserveincomes$ is a linear function of the number of consumers in the system.

Dual to the dollar reserve, token reserve $\tokenreserve$ increases with buy backs and decreases with payments made to the service providers, i.e.,
\begin{equation}\label{eq:reserve_tokens}
    R_{t+1}^{\text{Token}} = \tokenreserve + \paytokens - \buybacktokens. 
\end{equation}

\subsubsection{Token Price}

The token price at time $t$ is given by $\tokenprice$, and we assume it is market clearing. This is to say that for supply $\totalsupply$ at time $t$ and demand $\demand$ at time $t$ we have,
\begin{equation*}
    \tokenprice = \frac{\demand}{\totalsupply}.
\end{equation*}
The demand for tokens is a (unspecified) function of the number of consumers in the system $\numconsumer$ and the price of the token $\tokenprice$. 
We can assume that for a fixed price, demand is porportional to the number of consumers, and therefore it is worth pointing out that for a fixed token price, $\reserveincomes \propto \demand$.

\begin{remark}
Vanilla buy back and pay strategies, such as those used in Helium, reach equlibria.
By ``vanilla,'' we mean a strategy entirely clearing its income at each timestep, i.e.,
\begin{align*} 
    \reserveincomes = \buybackdollars, && \paytokens = \buybacktokens.
\end{align*}
Then, by verifying equations (\ref{eq:supply}--\ref{eq:reserve_tokens}) one sees that the circulating supply remains invariant, $\totalsupply = S_{t-1} = \ldots = S_0$, and the reserves $\dollarreserve$ and $\tokenreserve$ will remain at their initial value of zero as well.
\end{remark}



\subsubsection{State, Control and Cost Variables:}

As mentioned in Section \ref{sec:controller}, we refer to the state and control variables symbollically as $x_t$ and $u_t$ respectively. Informed by the previous discussions, these variables are given by
\begin{align*}
    \state{t} = \begin{bmatrix}
            \totalsupply, & \dollarreserve, & \tokenreserve, & \tokenprice
        \end{bmatrix}^{\top}, &&
    \control{t} = \begin{bmatrix}
            \buybackdollars, & \paytokens & \incentive \end{bmatrix}^{\top}.
\end{align*}
Additionally, as our method is {\em predictive} we use forecasts predicting the future state of the system.
In particular, we assume access to forecasts on the future demand and income which could be obtained via estimation, crowdsourcing, or other techniques.
The forecasts at time $t$ are,
\begin{equation*}
    \forecasted{t} = \begin{bmatrix}
            \widehat{\demand}, & \widehat{\reserveincomes}
        \end{bmatrix}^\top.
\end{equation*}

Now we can fully write the nonlinear dynamics of our system, captured by $f:\state{t},\control{t},\forecasted{t}\mapsto \state{t+1}$, using Equations (\ref{eq:supply}--\ref{eq:reserve_tokens}):
\begin{equation}\label{eq:dynamics}
    \state{t+1} = f(\state{t}, \control{t}, \forecasted{t}) =
    \begin{bmatrix}
        x_{t}(0) + u_{t}(1) - \frac{u_t(0)}{x_t(3)+u_t(2)} \\
        x_{t}(1) + s_{t}(1) - u_{t}(0) \\
        x_{t}(2) + \frac{u_t(0)}{x_t(3)+u_t(2)} - u_{t}(1) \\
        \frac{s_{t+1}(0)}{x_{t+1}(0)}  
    \end{bmatrix}.
\end{equation}

\subsubsection{Cost Function}
We let the cost function be given by the sum of the square errors between reference trajectories for state $\tokenprice$ and control variables $\buybackdollars$ , $\paytokens$. This is,
\begin{equation}\label{eq:cost}
    J(x_0,u_{0:H-1}) = \mathlarger{\mathlarger{\sum}}_{t=0}^{H}
\begin{bmatrix}
    \beta_1 \\ \beta_2 \\ \beta_3
\end{bmatrix}^\top
\begin{bmatrix}
    \left( x_t(3) - \bar{x}_t(3) \right)^2 \\
    \left( u_t(0) - \bar{u}_t(0) \right)^2 \\
    \left( u_{t}(1) - \bar{u}_t(1) \right)^2
\end{bmatrix},
%        \beta_1 \left( x_t(3) - \bar{x}_t(3) \right)^2 + \beta_2 \left( u_t(0) - \bar{u}_t(0) \right)^2 + \beta_3 \left( u_{t}(1) - \bar{u}_t(1) \right)^2,
\end{equation}
where the social planner's choice of $\beta_1, \beta_2$, and $\beta_3$ control the tradeoffs between prioritizing one reference trajectory over others.
\subsection{Formal Control Problem}\label{subsec:control_problem}

Now, using Equations (\ref{eq:dynamics}) and (\ref{eq:cost}) we can write finally the formal control problem:

\begin{equation}\label{eq:formal_problem}
\begin{array}{ll@{}ll}
    \underset{u_{0:H-1}}{\text{minimize}} & \underset{s_{0:H-1}}{\mathbb{E}}\big[J(x_0,u_{0:H-1}; s_{0:H-1})\big], &&\\
    \text{subject to}\;\;&x_{t+1} = f(x_t, u_t, s_t) \quad & \forall t \in \{0, \dots, H-1\} & \\
                         & x_{t} \in \mathcal{X} & \forall t \in \{0, \dots, H\} & \\
                         & u_{t} \in \mathcal{U} & \forall t \in \{0, \dots, H-1\} & \\ 
\end{array}
\end{equation}

\begin{remark}
This is a nonlinear (and possibly nonconvex) program.
However, due to the smooth dynamics and quadratic cost function the iterated linear quadratic regulator (iLQR) and sequential convex programming (SCP) are great fits for solving problem (\ref{eq:formal_problem}).
\end{remark}


\subsection{Market Dynamics}

Now we will more fully expouse the market dynamics arising from the selfish behavior of rational consumers.
We interpret each timestep as a two step sequential game of complete information between two distinguished parties: The consumers and the controller, where the controller seeks to optimize program (\ref{eq:formal_problem}) and the consumers seek to maximize the value of their token holdings over the time horizon.
By complete information, we mean that facts about the opponent respectively are common knowledge.
This is to say that consumers are aware of the controller's forecasts and reference trajectories.
We also assume that our information regarding the market price and supply is perfect and common knowledge.

Suppose the controller moves first by posting a price $(\tokenprice + \incentive)$.
The consumers respond by selling an $\alpha_t$-fraction of their collective holdings, where $\alpha_t$ is chosen in the following way:
The value of the consumers' holdings at timestep $t$ is a sum of the price they can get {\em today} and the price they can get {\em tomorrow}.
This is to say, that the consumer utility $U_t$ in dollars at time $t$, as a function of the game strategies, is given by,
\begin{equation*}
    \utility = \underbrace{\alpha_t \cdot\totalsupply(\tokenprice+\incentive)}_{\substack{\text{Current earnings from selling} \\ \text{ $\alpha_t$-fraction of supply.}}}  + \underbrace{(1-\alpha_t) \cdot \gamma \totalsupply \mathbb{E}(p_{t+1}^{\text{Tok}})}_{\substack{\text{Future expected earnings from} \\ \text{holding $\alpha_t$-fraction of supply.}}}.
\end{equation*}
In the above, it is worth noting that $\gamma$ is a risk factor attenuating the expected future earnings from not selling.
Furthermore, the randomness in the expectation is due to noise present in the forecast as our controller is not randomized.

So, in the game the optimal consumer strategy, which is to say their choice of $\alpha_t$, is given by the following:
\begin{equation}\label{eq:consumer_strategy}
    \max_{\alpha_t \in [0,1]}U_t(\alpha_t, \incentive).
\end{equation}
Moreover, due to program (\ref{eq:consumer_strategy}), the controller can compute the consumer strategy for any incentive price $\incentive$.
This means that we can transition the control problem (\ref{eq:formal_problem}) into the setting with incentives by constraining the amount of tokens the controller can buyback by a function of the consumer strategy,
\begin{equation*}
    \buybacktokens \leq \alpha_t \cdot \totalsupply,
\end{equation*}
where $\alpha_t$ is computed as a function of incentive price through program (\ref{eq:consumer_strategy}).
This means that in practice the controller can account for selfish behavior through roll out simulations to identify good incentive prices.
However, what would be even better is if the controller could play optimally by identifying the incentive price $\incentive^*$ inducing the Nash equilibrium maximizing program (\ref{eq:formal_problem}), $(\alpha_t^*, \incentive^*)$.
This makes a bilevel optimization problem with which our framework affords us the ability to make strong analytical statements.
This is, in the sequel we examine the existence of Nash equilibria in this game, as well as the {\em price of anarchy} which bounds the largest gap between the objective value the controller obtains in the setting with and without incentives.

\iffalse
\subsection{Controller}

In this section we will describe our controller, in here we will assume that our controller is a adaptive to the price estimation and operates under the assumption that the market is a competitive market and the price of the token is a function of the demand and supply of the token. In addition to that the consumers are aware of the controllers target and try to optimize their utility which is a amount of dollars they can get from the system.
Thus the optimization problem for the controller can be defined as:

\begin{small}
    \begin{align}
        \min_{\incentive, \paytokens, \buybackdollars} &  c_f(p^{\text{Token}}_H) + \sum_{t=0}^H c_t(\tokenprice,\incentive,\paytokens,\buybackdollars) \\
        \text{s.t.} & S_{t+1} = \totalsupply + \buybacktokens - \paytokens  \forall \hspace{1mm} t = 0, \ldots, H-1  \\
        & R_{t+1}^{\text{Token}} = \tokenreserve + \paytokens - \buybacktokens \\
        & R_{t+1}^{\text{USD}} = \dollarreserve - \buybackdollars + \reserveincomes \\
        & \tokenprice = \frac{\demand}{\totalsupply} \\
        & \buybackdollars \geq 0 \\
        & \paytokens \geq \frac{\beta_t \times \reserveincomes}{\tokenprice} \\
        & \buybacktokens \leq \alpha_t \times \totalsupply \times (\tokenprice + \incentive) \\
        & \alpha_t \in \arg\max_{\alpha_t} \utility \\
        & \text{s.t.}  \alpha_t \in [0,1] 
    \end{align}
\end{small}.
\fi




==> sections/old/sandeep_intro.tex <==
Today, we are seeing a surge in blockchain-based physical infrastructure networks, ranging from decentralized wireless, to storage/compute, and electric vehicle charging networks. For example, Helium and Pollen are two prominent decentralized wireless networks (DeWi) that reward the general public to build, maintain, and send data over 5G hotspots. Similarly, projects such as FileCoin offer decentralized file storage and compute services. These networks reward suppliers in a cryptocurrency token to build, secure, and offer valuable services on the infrastructure network. Likewise, consumers can exchange US dollars (USD) for tokens, which allow them to use the infrastructure network’s services. 

Despite the rising popularity of decentralized infrastructure networks, we lack systematic tools to design their token economies to incentivize supply growth and consumer demand. Today’s token economies largely target financial services, such as Bitcoin and Ethereum, and often operate with a fixed supply of tokens. However, these fixed supply systems are starkly different from physical infrastructure networks. For example, in a fixed supply system such as Bitcoin, early adopters can hoard tokens since they are scarce and valuable. Moreover, late adopters might be dis-incentivized to join or maintain the network since token rewards could be smaller compared to early investors. 

\input{fig_latex/fig1_overview_diagram.tex}

Our central thesis is that a token economy should continually incentivize new suppliers to join the blockchain and provide ubiquitous services, such as 5G connectivity for Helium or even electric charging stations for Tesla’s new TeslaCoin. As such, the number of tokens should gracefully scale with the size of the blockchain network, which we cannot know a-priori. However, continually rewarding suppliers with newly created tokens can lead to inflation if such payments are not delicately balanced
with the consumer demand for infrastructure services. To solve such problems, a number of projects have recently proposed a ``burn-and-mint'' token economics (tokenomics) model, where a central reserve ``mints'' tokens to reward suppliers, while tokens are ``burnt'' (deleted from the circulating supply) when consumers want to use network services. By adaptively burning tokens, we can reduce the token supply to reach a supply and demand equilibrium. 

Moreover, the burn-and-mint equilibrium (BME) needs to be ``programmable'' so that  blockchain-based infrastructure networks can maximize the total utility of all users. For example, this network utility function (performance criterion) can include maintaining a stable, steadily growing token price with low volatility. Likewise, this network cost function can incentivize new suppliers/consumers to expand geographical coverage. Moreover, the BME-based token economy might always need to satisfy
strict performance guarantees and constraints, such as limiting the number of tokens minted or burned per day. 
%or always need to keep a minimum amount of tokens in a central treasury. 
%For example, we might limit the number of tokens minted or burned per day or always need to keep a minimum amount of tokens in a central treasury. 

Our key insight is that token economies can be modeled as dynamical systems, which allows us to leverage powerful ideas from \textbf{mathematical control theory} to maximize a blockchain network’s utility function. Control theory is a natural tool since the token economy is a dynamical system – the circulating token supply, token price, and consumer demand change as a function of our burn and mint decisions. Likewise, we have control authority – we can adapt how we burn or mint to regulate the token economy. Moreover, we can design a control cost function that captures key metrics for desired blockchain performance and evolution of the blockchain dynamical system. Crucially, we can model the dynamics of the system, since we engineer the blockchain protocol and token economy dynamics. As such, regulating the blockchain token economy is a model-based control problem, which can be solved using powerful ideas from nonlinear optimization and optimal control theory. 

In essence, the contributions of this paper are three-fold: 
To the best of our knowledge, we are the first to apply optimal control theory to design blockchain token economies. 
We introduce a general dynamical systems theory for blockchain token economies that can flexibly model fixed supply as well as burn-and-mint systems, along with various network cost functions. 
We design a control system for a token economy using nonlinear model predictive control (MPC) methods that are used in high-performance, safety-critical applications like autonomous driving \cite{williams2018information,bhardwaj2022storm}, robotic manipulation, and rocket guidance \cite{agrawal2020learning}. We demonstrate these methods beat common heuristic controllers, such as proportional integral derivative (PID) controllers used by some algorithmic stablecoins. Specifically, we beat PID by $X\times$ on simulated network growth pattern datasets. Further, we beat
heuristic controllers by $Y\times$ on real network time series growth patterns from the Helium DeWi blockchain. 
We introduce a novel game-theoretic formulation that captures how owners of tokens and a central reserve strategically interact to maximize overall network welfare.



==> sections/old/strategic.tex <==
\textcolor{red}{Any game analysis should go here.}

\input{fig_latex/fig2_game}

As a cost function we will use quadratic cost function with respect to the price reference and thus the cost function becomes:

\begin{small}
    \begin{align}
        \cost = \frac{1}{2} \times \alpha \times (\tokenprice - \pricereference)^2
    \end{align}
\end{small}.

In here we will assume that the token holders are intelligent and they are aware of the controllers target and they are trying to maximize their utility in each time step.
so they select the maximium amount of token to sell in each time step to maximize their utility. Thus this problem can be posed as bilevel optimization problem. The controller problem is non-convex but coin holders problem is convex and we can solve it using the standard convex optimization techniques. for the optimal $\alpha$ we will assume that the KKT conditions hold.
Thus we canreplace the controller problem with the following problem:

\begin{small}
    \begin{align}
        \min_{\incentive, \paytokens, \buybackdollars} &  c_f(p^{\text{Token}}_H) + \sum_{t=0}^H c_t(\tokenprice,\incentive,\paytokens,\buybackdollars) \\
        \text{s.t.} & S_{t+1} = \totalsupply + \buybacktokens - \paytokens  \forall \hspace{1mm} t = 0, \ldots, H-1  \\
        & R_{t+1}^{\text{Token}} = \tokenreserve + \paytokens - \buybacktokens \\
        & R_{t+1}^{\text{USD}} = \dollarreserve - \buybackdollars + \reserveincomes \\
        & \tokenprice = \frac{\demand}{\totalsupply} \\
        & \buybackdollars \geq 0 \\
        & \paytokens \geq \frac{\beta_t \times \reserveincomes}{\tokenprice} \\
        & \buybacktokens \leq \alpha \times \totalsupply \times (\tokenprice + \incentive) \\
        & \lambda_i \geq 0 \\
        & \lambda_1 \times (1-\alpha) = 0 \\
        & \lambda_2 \times (-\alpha) = 0 \\
        & \alpha \geq 0 \\
        & \alpha \leq 1 \\ 
        & \Delta_\alpha \utility - \lambda_1 - \lambda_2 = 0 \\ 
    \end{align}
\end{small}.

Which we can solve with sequential convex programming (SCP). Therefor we can solve the bilevel optimization problem with the following steps:

\begin{algorithm}[H]
\caption{Bilevel Optimization Problem}
\label{alg:scp}
\begin{algorithmic}[1]
\STATE \textbf{Input:} $H$, $\alpha$, $\beta$, $\gamma$, $\pi$, $\tokenprice$, $\pricereference$, $\reserveincomes$, $\reservepayments$, $\numconsumer$, $\numproducer$, $\productprice$, $\tokenreserve$, $\dollarreserve$, $\totalsupply$
\STATE \textbf{Output:} $\incentive$, $\paytokens$, $\buybackdollars$
\STATE \textbf{Initialize:} $\alpha = 0.5$, $\lambda_1 = 0$, $\lambda_2 = 0$
\STATE \textbf{for} $t = 0$ \textbf{to} $H$ \textbf{do}
\STATE \hspace{1mm} $\lambda_1 = \lambda_1 + \alpha \times \Delta_\alpha \utility$
\STATE \hspace{1mm} $\lambda_2 = \lambda_2 - \alpha \times \Delta_\alpha \utility$
\STATE \hspace{1mm} $\alpha = \alpha + \lambda_1 \times (1-\alpha) + \lambda_2 \times (-\alpha)$
\STATE \hspace{1mm} $\alpha = \max(0, \min(1, \alpha))$
\STATE \hspace{1mm} $\Delta_\alpha \utility = \frac{1}{2} \times \alpha \times (\tokenprice - \pricereference)^2$
\STATE \hspace{1mm} $\incentive = \alpha \times \Delta_\alpha \utility$
\STATE \hspace{1mm} $\paytokens = \frac{\beta_t \times \reserveincomes}{\tokenprice}$
\STATE \hspace{1mm} $\buybackdollars = \alpha \times \totalsupply \times (\tokenprice + \incentive)$
\STATE \hspace{1mm} $\buybacktokens = \buybackdollars \times \frac{\tokenreserve}{\dollarreserve}$
\STATE \hspace{1mm} $\tokenreserve = \tokenreserve + \paytokens - \buybacktokens$
\STATE \hspace{1mm} $\dollarreserve = \dollarreserve - \buybackdollars + \reserveincomes$
\STATE \hspace{1mm} $\totalsupply = \totalsupply + \buybacktokens - \paytokens$
\STATE \hspace{1mm} $\tokenprice = \frac{\demand}{\totalsupply}$
\STATE \hspace{1mm} $\pricereference = \pi \times \tokenprice$
\STATE \hspace{1mm} $\reserveincomes = \gamma \times \reservepayments$
\STATE \hspace{1mm} $\reservepayments = \numconsumer \times \productprice + \numproducer \times \tokenprice$
\STATE \hspace{1mm} $\demand = \numconsumer \times \productprice + \numproducer \times \tokenprice$
\STATE \textbf{end for}
\end{algorithmic}
\end{algorithm}

